Extending Wire-Driven Parallel Robots to Multi-Floating-Link Systems with an Inter-Body Wire

Parallel wire-driven systems are a framework in which multiple wires are connected to an end effector, and the end effector is driven by the tensions of those wires. Because they can transmit large forces, up to the breaking strength of the wires, over lengths on the order of several tens of meters, they can realize powerful actuation in large workspaces. In recent years, studies have also investigated connecting wires to external environments such as trees and columns and forming parallel wire actuation on site. However, conventional parallel wire-driven systems often assume a single end effector, and because of interference between wires and links in a shared workspace, it has been difficult to handle multiple floating links simultaneously. In this study, we realize multi-floating-link parallel wire actuation by introducing an inter-body wire. In real-robot experiments, the two bodies supported and lifted a mannequin and transferred it onto a stretcher as a rescue motion. This shows that parallel wire actuation can be extended from a single end effector to a multi-floating-link system, and indicates its potential for broader tasks such as the manipulation of large objects and rescue support.

==> preamble.tex <==
%
%
\providecommand{\PDFAUTHOR}{}
\providecommand{\PDFKEYWORDS}{}
\providecommand{\PDFSUBJECT}{}
\providecommand{\PDFTITLE}{}

\RequirePackage[l2tabu, orthodox]{nag} %
\usepackage[all, warning]{onlyamsmath} %
\usepackage{color}
\usepackage[bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
     colorlinks=true,%
     linkcolor=black,%
     citecolor=black,%
     urlcolor=black,%
     bookmarksopen=true,%
%
     pdftitle=\PDFTITLE,%
     pdfsubject=\PDFSUBJECT,%
     pdfauthor=\PDFAUTHOR,%
     pdfkeywords=\PDFKEYWORDS]{hyperref}
%


\usepackage{url} %
%
\usepackage{txfonts,mathptmx}

%

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}


%
\usepackage[figure,figure*,table,table*]{hypcap}
\usepackage{eclbkbox}
%

\usepackage{url} %
%
%
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\algblockdefx{FORP}{ENDFORP}[1]%
  {\textbf{for}#1 \textbf{do in parallel}}%
  {\textbf{end for}}
\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}
%
%
%

%
%
%
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\subsecref}[1]{Subsection \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
%
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}
%
%

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

\newcommand{\ctext}[1]{\raise0.2ex\hbox{\textcircled{\scriptsize{#1}}}}

